Dynamic optimal congestion pricing in multi-region urban networks by application of a Multi-Layer-Neural network

Traffic management by applying congestion pricing is a measure for mitigating congestion in protected city corridors. As a promising tool, pricing improves the level of service in a network and reduces travel delays. However, real-world implementations are restricted to static pricing, i.e., the price is fixed and not responsive to the prevailing regional traffic conditions. Dynamic pricing overcomes these limitations but also affects the users route choices. This work uses dynamic pricing's influence and predicts pricing functions to aim for a system optimal traffic distribution. The framework models a large-scale network where every region is considered homogeneous, allowing for the Macroscopic Fundamental Diagram (MFD) application. We compute Dynamic System Optimum (DSO) and a Quasi Dynamic User Equilibrium (QDUE) of the macroscopic model by formulating a linear optimization problem and utilizing the Dijkstra algorithm and a Multinomial Logit model (MNL), respectively. The equilibria allow us to find an optimal pricing methodology by training Multi-Layer-Neural (MLN) network models. We test our framework on a case study in Zurich, Switzerland, and showcase that (a) our neural network model learns the complex user behavior and (b) allows predicting optimal pricing functions. Results show a significant performance improvement when operating a transportation network in the DSO and highlight how dynamic pricing influences the user's route choice behavior towards the system optimal equilibrium.

==> not_need_text_parts.tex <==

%% from related work and intro
Although optimal pricing solutions could be applied in the field, the users elasticities to a specific toll is not considered. The concept of elasticity gives the relation between the percentage of change in the demand and change in price. Hence, the quantities give insights to the reaction of users to a specific toll price. \cite{ref:Olszewski2005} derived the elasticity of different pricing systems (e.g., specific bridge sections in New York, motorways in Spain, cordon pricing in Singapore). The results indicate that elasticity is dependent on the type of pricing system (road section, specific infrastructure type, cordon), time of the day, and also if all or specific vehicles are priced. \cite{ref:Sarlas2013} extended the findings with an analysis in Athens (Greece). To this end, if the elasticities of users in the system are available, the concept can be utilized to determine optimal toll prices, if the following information is present: the DSO and QDUE of the transportation network for a known exogenous demand are known and hence allows the calculation of the system-, and user-optimal transfer flows. 

Different system designs such as (a) the pricing of one lane (High-Occupancy-Lanes) on a road segment (b) tolls for specific road segments and (c) tolls at the border of protected regions have been shown as beneficial. All mentioned methodologies find their place already in the field, where this work focuses on fixed corridor (or cordon) pricing systems applied in e.g., London, Stockholm or Singapore (a hybrid of facility-based tolls and cordons). The evaluation of cordon pricing systems show a decrease in the Vehicle Kilometers Traveled (VKT) and therefore are beneficial for the transportation network performance. Nevertheless, most of the pricing schemes are fixed over time and do not adjust to current traffic states (i.e., the current vehicle accumulations) in a system. The most advanced cordon pricing system so far is implemented in Singapore, where tolls are revised four times a year by evaluating the deviation of speed measurements.

appears simple: If users travel through a network from origin to destination, external costs are caused that they are not charged for. This includes e.g., the travel delay caused to others or the impact on the environment. As the external costs are proportional to traffic demand, their magnitude is higher in peak-hour traffic. Consequently, an optimal pricing function should capture this relationship.

%% elasticity pricing chapter

First, we introduce the concept of elasticity $E$ which can be defined by the fraction of partial derivative of demand $Q$ and price $P$ (at any point) and the product of price-demand ratio:
\begin{equation}
    E = \frac{\partial Q}{\partial P} \frac{P}{Q}.
\end{equation}
\cite{ref:Olszewski2005} have further introduced a simplified calculation of elasticities by utilizing the arithmetic average of demand and price quantities before and after a price change (i.e., mid-point elasticity). Hence, the elasticity can be derived by
\begin{equation}
\label{eq:ela}
    E = \frac{(Q_2 - Q_1)(P_2 + P_1)}{(P_2 - P_1)(Q_2 + Q_1)},
\end{equation}
where variables with index $1$ and $2$ represent demands and prices before and after the price change, respectively. We modify this concept for our problem by modeling the demand with transfer flows $M_{IH}(k)$, i.e., the flows that want to leave from region $I$ towards their destination $J$ and have to decide on which region to traverse based on the current costs and travel times. Hence, all transfer flows that leave a region $I$ and traverse via region $H$ are defined as:
\begin{equation}
    M_{IH}(k) = \sum_{J \in \mathcal{R}} M_{IHJ}(k).
\end{equation}
The price that a user has to pay for the travel is represented by the generalized cost matrices $C_{\mathrm{UE}}(k)$ and $C_{\mathrm{SO}}(k)$ for the DUE and DSO, respectively. Therefore we utilize (\ref{eq:ela}) and modify it to:
\begin{equation}
\label{eq:ela_mod}
    E(k) = \frac{\Big(M_{IH\mathrm{SO}}(k) - M_{IH,\mathrm{UE}}(k)\Big)\Big(C_{\mathrm{SO}}(k) + C_{\mathrm{UE}}(k)\Big)}{\Big(C_{\mathrm{SO}}(k) - C_{\mathrm{UE}}(k)\Big)\Big(M_{IH,\mathrm{SO}}(k) + M_{IH,\mathrm{UE}}(k)\Big)}.
\end{equation}
Note that the indices $\mathrm{SO}$ and $\mathrm{UE}$ represent the corresponding quantities computed by DSO and QDUE, respectively. If the elasticity matrix $E(k)$ is assumed as known and DSO has already been computed by the proposed methodology from Section~\ref{sec:eq_derivation}, we can rearrange (\ref{eq:ela_mod}) to derive the new cost matrix $C_{\mathrm{P}}(k)$, which denotes the generalized costs that users need to experience so that system optimum is achieved. 
\begin{equation}
\label{eq:ela_mod2}
    C_{\mathrm{P}}(k) = \frac{C_{\mathrm{SO}}(k)\Big (M_{IH,\mathrm{UE}}(k)\Big (E(k)+1\Big ) + 
M_{IH,\mathrm{SO}}(k) \Big (E(k)-1\Big )\Big )}{M_{IH,\mathrm{UE}}(k) \Big (E(k)-1\Big ) + M_{IH,\mathrm{SO}}(k) \Big (E(k)+1\Big )}.
\end{equation}

Finally, we can derive the tolls matrix $P(k)$ which contains all toll prices $p_{IH}(k)$ by subtracting the generalized cost matrix $C_{\mathrm{P}}(k)$ from $C_{\mathrm{UE}}(k)$
\begin{equation}
    P(k) = C_{\mathrm{P}}(k) - C_{\mathrm{UE}}(k).
\end{equation}
Note that the elements of $P(k)$ are not bounded by any means, and in that sense can give not only extremely high but also negative prices, which means that there should be an economic incentive for people to travel through this toll (so that the systems operates in DSO). Nevertheless, in practice, the derived prices are bounded by operational constraints, e,g,\ by following condition:
\begin{equation}
    p_{\min} \leq p_{IH}(k) \leq p_{\max}, \ \forall p_{IH}(k) \in P(k),
\end{equation}
where $p_{\min}$ denotes the minimum permissible price, which should be set to 0 for practical reasons and $p_{\max}$ denotes the maximum permissible price, dependent on the, e.g., each country's currency or gross domestic product. Note that the smaller the space for all elements $p_{IH}(k)$ is chosen, the bigger the deviation from the DSO will be.

\begin{table}[tb]
\centering
\caption{TS comparison and corresponding improvement of QDUE and DSO scenarios for $R_1$ -- $R_4$, respectively. CS denotes the time a region experienced congestion; NCS the time a region was non-congested; IMPR states the percentage of improvement from QDUE to DSO.}
\begin{tabular}{lrrr||rrr|r||}
\toprule
  & QDUE  & CS & NCS  &  DSO & CS & NCS  & IMPR \\
  & [veh$\cdot$h]$\cdot$10$^6$ & [h] & [h] & [veh$\cdot$h]$\cdot$10$^6$ & [h] & [h] & [\%] \\
 \midrule
$TS_1$             & 1.79           & 0.15       &      0.68    &  1.40     &   0.13      & 0.70       & 21.93          \\
$TS_2$             & 2.30          & 0.00      & 0.83         & 2.10    & 0.00       & 0.83        & 8.77         \\
$TS_3$            & 2.77           & 0.00          & 0.83        &  2.65     & 0.00          & 0.83      &  4.39         \\
$TS_4$            &  1.94          & 0.00          & 0.83       &   1.65   & 0.00          & 0.83       & 14.99  \\ 
$TTS$ [veh$\cdot$h]$\cdot$10$^6$   &  31.18    & -&-&  23.89 &-&-   & 23.38  \\ 
$TTD$ [veh$\cdot$km]$\cdot$10$^6$  &  54.23    & -&-&  49.96 &-&-  &  7.87   \\
\bottomrule
\end{tabular}
\label{tab:performance_comparison}
\end{table}

%\begin{table}[!b]
%\centering
%\caption{Toll activation time for all $T_{IH}$ relative to the simulation time in %[\%].}
%\begin{tabular}{lrrrr}
%\toprule
%$T_{IH}$ [\%] & $H = 1$      & $H = 2$      & $H = 3$      & $H = 4$      \\
%\midrule
%$I = 1$ & NA          & 70.59  & 21.00  & 34.45  \\
%$I = 2$ & 50.59  & NA          & 52.27  & 42.19  \\
%$I = 3$ & 5.04   & 49.75  & NA          & 7.56   \\
%$I = 4$ & 3.36   & 48.91  & 22.69  & NA   \\
%\bottomrule
%\end{tabular}
%\label{tab:toll_final2}
%\end{table}

%Finally, we compute the space mean speed $V$ of the network defined as

%\begin{equation}
%    V = \frac{TTD}{TTS}.
%\end{equation}

For this case study, we have applied the procedure offline and derived the toll matrix that should be applied to the modeled QDUE.  For the elasticity, we define a normal distribution $\mathcal{N}(-0.106,0.01)$, where the mean value is based on findings from Singapore cordon pricing system in~\cite{ref:Olszewski2005}. We assume that all users react to toll prices with the same mean elasticity of $-0.106$ and consider the quantity as constant.


Consequently, we derive the transfer flows for DSO and QDUE for all time steps $k$, respectively; i.e, $M_{IH,\mathrm{SO}}$ and $M_{IH,\mathrm{UE}}$. By applying the equations for deriving the price matrix $P$ for all timestamps $k$ all toll functions are computed. It is assumed that a toll is applied to every vehicle traversing any region border. Figure~\ref{fig:tolls_wo_constraints} shows all the derived prices over time for all regions ($R_1$ -- $R_4$), i.e., 12 dynamic pricing functions are determined. As in practice, a toll is not changing its price every second; we show the average price for every $100$ [s].

The pricing functions show some impracticable behavior, because of: (a) negative prices occur which means that the route via the nodes $I$ and $H$ should have more traffic volume then the system currently serves (i.e., users should experience a cost reduction to get an incentive to chose the route); (b) the pricing functions show fluctuations where very high positive and negative prices occur, which occurs because the derivation of the cost matrix produces very high outputs if the deviation between QDUE and DSO is small. If we determine the deviation of vehicle accumulation between QDUE and DSO in Figure~\ref{fig:acc_final} in $R_1$ -- $R_4$ at the time step, where the price fluctuations occur, one can note that the absolute magnitude of the quantity becomes small.

